Bringing the second quantum revolution into high school

The aim of this thesis is to bridge the gap between the world of physics research and secondary education on contemporary quantum physics. We fostered the creation of a generative learning environment formed by quantum physics researchers, high school physics teachers and student. The result was the development of an teaching approach to the core ideas of quantum physics (quantum states, superposition and measurement) that has been used to design and implement teaching-learning activities in regular high school lessons.

==> Stuff.tex <==

%%%%%%%%%%%%%%%%%%%% STUFF %%%%%%%%%%%%%%%%%
%%%%%%%%% chap LET carcano + chiara %%%%%%

\begin{comment}
Alla fine del percorso i docenti hanno deciso di somministrare un questionario con l'obiettivo di valutare gli apprendimenti, in particolare la capacità degli studenti di applicare quanto appreso in un contesto simile. Il fenomeno preso in considerazione è stato quello della doppia fenditura fatta con un fascio di elettroni. Concettualmente simile, lo scopo era quello di vedere se gli studenti erano in grado di analizzare i risultati dell'esperimento facendo riferimento ai concetti di stato quantistico visti nelle lezioni.
I risultati non sono stati valutati in modo soffisfacente, permanendo delle criticità nel modo in cui gli studenti giustificano le loro scelte. 
Questo ha però dato l'occasione ai docenti di far emergere i dubbi rimasti e di continuare la discussione con gli studenti a partire proprio dalle loro difficoltà.
\end{comment}



%%%%%%%% inserire arfico likert con i risultati del quesito sul reticolo TQP_ElectronDiffraction_CARCANO_Apr21_elaborazione
%ExitTEST_DIFFRAZIONE

%quanto emerso nel PD per la 
%Stabilito che è possibile descrivere l'elettrone usando il linguaggio delle onde, il passo successivo 

%quando parliamo di onda parliamo di qualcosa che viene desfritto dalla soluzioen delle equazione delle onde
%l'ipoetsi di de Broglie viene dunque presentata come una speculazione fatta circa gli aspetti ondualtori degli elettroni che si manifestano nell'espeirmento e l'eqauoznr di Sch è presentata come l'equazione delle ond che permette di ricavare lo stato dell'elettrone nel suo proparagarsi nello spazio.

%Questa distinzione risulta importante allo scopo di facilitare il processo di meaning making ed è stata parte del lavoro sulla SMK4T e di ricostruzione dei contenuti per l'insegnamento sviluppato dalle docenti.

%%%%%%%%%% lo scopo qui nin è che gli stidenti sappiano usare il formalismo nel dettaglio ma che colgano l'ide acnhe la descrizione posibile del comportamneto dell'elettrine può esssere fata in termini molto astratta usando funzioni complesse. tale tipo di descrizione è sicuramente molto asyratta ma consente di ricostruire l'informazione sull'oggetto dal momento che quando vado a misurare ritrovo quanto è previsto dal modello. infatti tale modello prevede la formaizone degli anelli di diffrazione. Non siono in grado di descrivere come si muove l'elettrone così come faccio con le palline classiche, ma comuqneu posso ricavare info


%%%%%%%%%%% legame tra deBRogleie e schroedinger
\begin{comment}
La descrione in termini di onde proposta da DeBroglie è i
legame 

Esperimento e sua interpretazione
uso del laboratorio remotoi
Results
Confronto questionario pre post

usare lo stato permette di descriverlo
passata l'idea che 
%%%%% fatto fatica a raccogliere elementi diretti dagli studenti visto che l'attività è stata fatta a distanza. le quoting sono catturate dalle domande e dagli interventi presi durante l'intervento

%%%%% criticità nella raccolta dati e quindi meglio metere fuoco sui docenti%%%%%%%%%%%%%%%%
elemento critico: la raccolta diretta dei dati dagli studenti. l'interazione limitata con gli studenti non ha permesso di raccogliere tanti elementi di riflessione sull'acquizione dei concetti. nell0anakisi non ci siamo dunque concentrati sulla valutazione degli apprendimenti degli studenti ma sugli apsetti che gli insegnanti hanno individiuato come positivi o critivi rispetto al percorso propostp

%%%%%%%%%%%% aspetti positivi e negativi in base alla valitazione dei docenti
positivo 
fare esperimento e dare la possibilità di vedere i fenomeni e non solo limitarsi a parlarne,

\begin{quote} {\fontfamily{lmtt}\selectfont
    studenti contenti di essere in laboratorio, questo li motiva molto
}\end{quote}
usare quello per avviare la diuscussio ne

\begin{quote} {\fontfamily{lmtt}\selectfont
    anche in 
}\end{quote}

eleento positivo la determinazione dei docenti nel portare avanti i percorsi nonistabt le difficotlà logistiche e contestuali geenrati dlal'emergenza sanitaria. in questo senso risulta ancora più significativa la collavorazione tra diocenti e ricercatori (aver ad esempio condiviso le risorse del lab remoto o degli striumenti)

elemnto critico
il tempo poco per introdurre tanti concetti
uso della matematica che ancora crea ostacoli. 

% apsetto positivocurare meglio i momenti di assessment 

%%%% quote: se ho capito bene, quello che posso sapere, cioè che posso sempre conoscere è lo stato... cioè quella cosa che mi dice dove andrà a sbattere l'elettrone, poi dove realmente andrà lo posso vedere solo quando sbatte, cioè solo dopo [che ho fatto] la misura

%%%%%%% quote: faccio proprio fatica a capire cosa voglia dire

%%%%%%%% quote: l'elettrone è una particella perché quando lo vedo so dove è... (acquisito la necessità della misura per l'attribuzione di una proprietà)

%%%%%%%%%%%% A qualcuno ha aperto i chakra.
 
As reported by the teachers in their post-activity reflection, this experience also helped the students move from the idea of the electron as a “localized particle” to the concept of a “quantum object” that cannot be fully described as a classical spinning ball, but only in terms of a probability wave, solution of the Schrödinger’s equation, within the theoretical framework of Born’s interpretation of quantum mechanics (see also sec.\ref{sec:carcano})\\

%% commento studente di gabriella sul senso della funzione d'onda come tante onde sobrapposte, necessario quindi introdurre l'idea che il 

il fatto che posso scrovere lo stato dell'elettrone come sovrapposizione di stati ha chairto in qualche modo dhe non è che l'eettrone è un insieme di tante piccole onde che oscillano

%%%%%%%%%%%%%%%%%%%%%%%% carcano %%%%%%%%%%%%%%%
(see. Teachers guided students in the analysis of quantum experiments involving the measurement of electron spin states using the Stern-Gerlach apparatus and introducing quantum superposition and Heisenberg inequality.

\end{comment}

%%%%%%%%%%%%%%%%% parte sulla luce messo in pausa per essere messo nella parte con gli studenti %%%%%%%%%%%%%

\begin{comment}
%\subsection{Nature of light: classical and quantum models}\label{sec:chiara-giaimila}

La natura è complicata %ref al paper WHAT IS LIGHT?

L'intenzione del docente è stata quella di partire dalla indicazioni nazionali relative al curriculum di fisica \cite{MIUR2010_211} per la costruzione di un percorso che andasse a toccare le tappe fondamentali dello sviluppo della fisica contemporanea a partire dallo studio della radiazione elettromagnetica come teoria classica della luce.
Tra gli obiettivi vi è quello di affrontare la questione del dualismo onda particella che secondo il docente 
\begin{quote} {\fontfamily{lmtt}\selectfont
    spesso presentata in modo frettoloso sui libri di scienze. 
}\end{quote}

Si vuole quindi fornire agli studenti strumenti interpretaticvi dei fenomeni quantistici più efficaci per affrontarne gli aspetti più controintuitivi

Il percorso è struturato in tre differenti fasi
\begin{enumerate}
    \item le proprietà ondulatorie della radiazione elettromagnetica (equazioni di Maxwell, onde elettromagnetiche, polarizzazione, interferenza, diffrazione);
    \item fisica quantistica (effetto fotoelettrico, spettri atomici, lunghezza d’onda di de Broglie e onde di materia);
    \item elementi di meccanica quantistica (onde di probabilità, esperimento della doppia fenditura e principio di sovrapposizione).
\end{enumerate}

Si tratta di tre differenti unità di apprendimento che il docente ha affrontato in un arco temporale di circa tre mesi insieme ad un gruppo di 24 studenti dell'ultimo anno di liceo scientifico. Il docente ha progettato in modo autonomo i diversi momenti, elaborando strategie didattiche basate su un approccio sperimentale che presentano differenti vantaggi.

\begin{quote} {\fontfamily{lmtt}\selectfont
    L’intero percorso sfrutta una didattica di tipo laboratoriale in grado di far confrontare le concezioni degli studenti e le loro previsioni con le osservazioni sperimentali che, nel caso della fisica moderna, risultano spesso controintuitive e di difficile accettazione e costituiscono un ostacolo di apprendimento rilevante. Inoltre si ha il vantaggio di “avvicinare” gli studenti a fenomeni che non fanno parte della loro esperienza quotidiana e risultano quindi astratti e difficilmente comprensibili. [TeacherAR]
}\end{quote}

Questo modo di approcciare i cambiamenti paradigmatici necessari allo studio delle fisica quantistica consente secondo il docente di 
\begin{quote} {\fontfamily{lmtt}\selectfont accompagnare gradualmente gli studenti a scoprire i limiti del modello in uso e a convincerli della necessità di introdurre dei cambiamenti che
normalmente vengono accettati con grande difficoltà [TeacherAR]
}\end{quote}
Il percorso è dunque anche una occasione per il docente di indagare nelle pre-scientific conceptions degli studneti e cpire in che modo una maggiore consapevolezza dei meccanismi che generano le difficoltà possa aiutare a progettare attività efficaci.

\begin{quote} {\fontfamily{lmtt}\selectfont
le concezioni a priori degli studenti che
spesso sono formate nel corso degli studi di scienze e che possono ostacolare l’apprendimento.
}\end{quote}
Si tratta di concezioni che secondo il docente nascono per analogia con idee e rappresentazioni formali classiche attraverso cui 
\begin{quote} {\fontfamily{lmtt}\selectfont
     gli studenti creano molto facilmente modelli interpretativi che, se errati, possono ostacolare gli apprendimenti successivi
}\end{quote}

La grande competenza del docente nell'individuare gli strumenti metodologici ha permesso di realizzare differenti tipologie di attività che hanno coinvolto in modo attivo gli studenti nella realizzazione di esperimenti. Attraverso l'uso di simulatori e la costruzioni di apparati sperimentali gli studenti hanno potuto raccogliere ed analizzare dati utili ad investigare concetti fondamentali della meccanica quantistica quali la quantizzazione dell'interazione luce - materia (effetto fotoelettrico) e lo studio degli spettri atomici.

\begin{figure}[hbt!]
    \centering
   \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{figure/ch6_40.png}
    \caption{Esempi delle attività svolte: a) grafico analisi dell'effetto fotoelettrico ottenuti combinando i dati del simulatore ricavati da gruppi differenti; b) spettrometro autocostruito; c) porzione spettro dell'elio otenuto da uno dei gruppi}
    \label{fig:Ch6_40_laboChiara}
\end{figure}

Il primo elemento verso per lo studio della natura degli oggetti quantistici è l'analisi dell'esperimento della diffrazione degli elettroni. L'attività è stata svolta come presentata nel Professional Development programme Quantum Jumps con modolità simili a quanto visto nel percorso precedente (see sec. \ref{sec:carcano}).
Al termine di questa prima fase gli studenti hanno quindi a disposizione i concetti di quantizzazione e dualismo che possono essere estesi anche allo studio della luce. Lo studio delle onde elettromagnetiche ha reso gli studenti 

\end{comment}
